You Can't Always Check What You Wanted: Selective Checking and Trusted Execution to Prevent False Actuations in Cyber-Physical Systems

Cyber-physical systems (CPS) are vulnerable to attacks targeting outgoing actuation commands that modify their physical behaviors. The limited resources in such systems, coupled with their stringent timing constraints, often prevents the checking of every outgoing command. We present a "selective checking" mechanism that uses game-theoretic modeling to identify the right subset of commands to be checked in order to deter an adversary. This mechanism is coupled with a "delay-aware" trusted execution environment (TEE) to ensure that only verified actuation commands are ever sent to the physical system, thus maintaining their safety and integrity. The selective checking and trusted execution (SCATE) framework is implemented on an off-the-shelf ARM platform running standard embedded Linux. We demonstrate the effectiveness of SCATE using four realistic cyber-physical systems (a ground rover, a flight controller, a robotic arm and an automated syringe pump) and study design trade-offs. Not only does SCATE provide a high level of security and high performance, it also suffers from significantly lower overheads (30.48%-47.32% less) in the process. In fact, SCATE can work with more systems without negatively affecting the safety of the system. Considering that most CPS do not have any such checking mechanisms, and SCATE is guaranteed to meet all the timing requirements (i.e., ensure the safety/integrity of the system), our methods can significantly improve the security (and, hence, safety) of the system.

==> Sections/optee_overhead_plot.tex <==

\subsection{Overhead of Various OP-TEE Components} \label{sec:optee_overhead}


\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.50]{smc_dist.pdf}
	\caption{Empirical CDF of execution times (y-axis) for checking actuation commands using TEE. The bottom right plot (last row) depicts the total context switch latency and the other plots show latency for individual TEE API components.} 
	\label{fig:sms_dist}
\end{figure}


Table~\ref{tab:smc_timing} shows the average latency of each of relevant OP-TEE APIs and Fig.~\ref{fig:sms_dist} illustrates the Empirical CDF of execution times. The empirical CDF is defined as
$
\widehat{F}_\beta(\hat{\kappa}) = \frac{1}{\beta} \sum_{i=1}^\beta \mathbb{I}_{[\hat{c}_i \leq \hat{\kappa}]},
$
where $\beta=10,000$ is the total number of experimental observations, $\hat{c}_i$ is computation time at the $i$-th experimental observation and $\hat{\kappa}$ represents the $x$-axis values (\ie execution times). The indicator function $\mathbb{I}_{[\cdot]}$ outputs $1$ if the condition $[\cdot]$ is satisfied and $0$ otherwise. Our measurements find that the total TEE context switch overhead in a Raspberry Pi platform is around $66$ ms. \hl{added the following statements} As a reference, many real-time tasks require to finish computation by $10$--$1000$ ms~\cite{lesi2017network, uav_flight_control,nemer2006papabench}. Hence, requiring $66$ ms to check a single actuation command can significantly limit the number of actuation commands a task can check in a Raspberry Pi-based system (while guaranteeing its timing requirements).  \hl{end}



\begin{table}[!t]%[!htb]
	\caption{Overhead of Checking Actuation\textsuperscript{*}}
	\label{tab:smc_timing}
	\centering
	\begin{tabular}{P{4.00cm} P{1.70cm}}
		\hline
		\bfseries API & \bfseries Latency ($\boldsymbol\mu$s)\\
		\hline
		\hline 
		\texttt{TEEC\_InitializeContext()} & $64$ \\
		\texttt{TEEC\_OpenSession()} & $49233$ \\
		\texttt{TEEC\_InvokeCommand()} & $146$ \\
		\texttt{TEEC\_CloseSession()} & $15682$ \\
		\texttt{TEEC\_FinalizeContext()} & $29$ \\
		\hline
		Total overhead & $65154$ \\
		\hline 
	\end{tabular}
	\vspace*{-0.5em}
	\begin{flushleft}
		\scriptsize
		\textsuperscript{*}Measurements from a Raspberry Pi 3 platform running Linux and OP-TEE with a constant frequency (1.2 GHz). We used the Linux high resolution timer (\texttt{clock\_gettime()} function with \texttt{CLOCK\_PROCESS\_CPUTIME\_ID} clock). Each timing measurements (99\textsuperscript{th}-percentile latency) was obtained from $10,000$ samples. 
	\end{flushleft}
\end{table}




